TimeRewind: Rewinding Time with Image-and-Events Video Diffusion

This paper addresses the novel challenge of ``rewinding'' time from a single captured image to recover the fleeting moments missed just before the shutter button is pressed. This problem poses a significant challenge in computer vision and computational photography, as it requires predicting plausible pre-capture motion from a single static frame, an inherently ill-posed task due to the high degree of freedom in potential pixel movements. We overcome this challenge by leveraging the emerging technology of neuromorphic event cameras, which capture motion information with high temporal resolution, and integrating this data with advanced image-to-video diffusion models. Our proposed framework introduces an event motion adaptor conditioned on event camera data, guiding the diffusion model to generate videos that are visually coherent and physically grounded in the captured events. Through extensive experimentation, we demonstrate the capability of our approach to synthesize high-quality videos that effectively ``rewind'' time, showcasing the potential of combining event camera technology with generative models. Our work opens new avenues for research at the intersection of computer vision, computational photography, and generative modeling, offering a forward-thinking solution to capturing missed moments and enhancing future consumer cameras and smartphones. Please see the project page at https://timerewind.github.io/ for video results and code release.

==> sec/Figures/fig_10.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{sec/Figures/Experiments/Figure_supp_more_syn_1.pdf}
   \caption{More comparisons on synthetic turbulence video. Two scenes are presented, with sharpness comparisons in the first row and temporal consistency comparisons in the second row through $x$-$t$ slices. ConVRT exhibits smooth $x$-$t$ slice patterns, indicating superior temporal stability over TurbNet and TSR-WGAN. ConVRT consistently produces sharper edges across the overall and zoomed-in regions.}
   \label{fig:supp_syn_more_1}
\end{figure*}

==> sec/Figures/fig_6_abla_fuse.tex <==
\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{sec/Figures/Supp/Abla_Fuse.pdf}
    \caption{Illustration of different ways of integrating EMA to SVD architecture. (a) EMA-Down, only integrating EMA to down and middle blocks, (b) EMA-Up, only integrating  EMA to up and middle blocks, (c) EMA, our final design of integrating EMA to all down, middle, and up blocks of SVD architecture.}
   \label{fig:abla_fuse}
\end{figure}


==> sec/Figures/fig_8.tex <==

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{sec/Figures/Experiments/Figure_clip.pdf}
   \caption{CLIP text prompt selection. Left: LPIPS against CLIP loss during optimization. Right: correlation scores between CLIP loss and LPIPS sequences for each text prompt. Text 3 is the final choice due to its highest correlation scores.}
   \label{fig:clip_select}
\end{figure}

==> sec/Figures/fig_9.tex <==

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{sec/Figures/Experiments/Figure_abalation.pdf}
   \caption{Ablation study of sharpness and temporal coherence for proposed INR enhancements. Sharpness is evaluated in the top row, temporal consistency in the bottom via $x$-$t$ slices. Column (a) introduces the base of ConVRT model, columns (b) and (c) show sharpness and detail improvements from Real-ESRGAN and CLIP, respectively, and column (d) confirms temporal stability gains from the temporal consistency regularization.}
   \label{fig:abala}
\end{figure*}



==> sec/Figures/figure_11.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{sec/Figures/Experiments/Figure_supp_more_real_1.pdf}
   \caption{More comparisons on real-world turbulence video. Two scenes are presented, with sharpness comparisons in the first row and temporal consistency comparisons in the second row through $x$-$t$ slices. }
   \label{fig:supp_real_more_1}
\end{figure*}

==> sec/Tables/table_1.tex <==
\begin{table}[t]
\centering
\vspace{-3pt}
\caption{Evaluation metrics tested on video with synthetic turbulence. \(\uparrow\): higher is better, \(\downarrow\): lower is better.}

\label{table:runtime}
\vspace{-2pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}cccccc@{}}
\toprule
Method           & \textbf{PSNR$_{Img}$ $\uparrow$} & \textbf{SSIM} $\uparrow$  & \textbf{LPIPS} $\downarrow$  & \textbf{E$_{warp}$} $\downarrow$ & \textbf{PSNR$_{x-t}$} $\uparrow$ \\ \hline 

Turbnet \cite{mao2022single}        & 21.977           & 0.708            & 0.279             & 0.0057           & 22.23   \\
TSRWGAN \cite{jin2021neutralizing} & 21.993           & 0.720            & 0.277             & 0.0026           & 22.40   \\
Ours                               & \textbf{22.383}  & \textbf{0.729}   & \textbf{0.255}    & \textbf{0.0024}  & \textbf{22.95}  \\
\bottomrule 
\label{table:syn}
\end{tabular}%
}
\end{table}
\vspace{-8pt}



==> sec/Tables/table_2.tex <==
\begin{table}[t]
\centering
\vspace{-3pt}
\caption{Ablation Study : The table presents PSNR$_{\text{img}}$, SSIM, LPIPS, E$_{\text{warp}}$, and PSNR$_{x-t}$ scores, demonstrating the improvements achieved by each successive refinement, culminating in our proposed ConVRT method. (a), (b), (c), and (d) correspond to the respective indices in Fig \textcolor{red}{9}.}
\vspace{-2pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
Method                          & \textbf{PSNR$_{Img}$ $\uparrow$} & \textbf{SSIM} $\uparrow$  & \textbf{LPIPS} $\downarrow$  & \textbf{E$_{warp}$} $\downarrow$ & \textbf{PSNR$_{x-t}$} $\uparrow$ \\ \hline
TSRWGAN \cite{jin2021neutralizing} & 23.58 & 0.739 & 0.230  & 0.0026   & 23.77   \\ 
TurbNet \cite{mao2022single}       & 23.44 & 0.732 & 0.228  & 0.0057   & 23.54   \\ 
TurbNet+Real-ESRGAN \cite{wang2021real}  & 22.48 & 0.713 & 0.213  & 0.0074   & 22.67   \\ \hline
Base (a)                             & 24.91 & 0.781 & 0.209  & 0.0017  & 25.44    \\
\quad + Real-ESRGAN (b)                     & 24.88 & 0.782 & 0.204  & 0.0020  & 25.11    \\
\quad + CLIP (c)                     & 24.71 & 0.784 & 0.193  & 0.0014  & 25.40    \\
\quad + temp. consistency (d)          & 24.90 & 0.787 & 0.189  & 0.0014  & 25.73    \\
= Ours (ConVRT) (d)                  & \textbf{24.90} & \textbf{0.787} & \textbf{0.189}  & \textbf{0.0014}  & \textbf{25.73}   \\
\bottomrule 

\label{table:abala}

\end{tabular}%
}
\end{table}
\vspace{-8pt}

% LPIPS
% 0.2002, 0.2124, 0.1989, 0.1226, 0.3193, 0.2433, 0.1884, 0.1889
% 0.1924, 0.2237, 0.1957, 0.4560, 0.2588, 0.2393, 0.1790, 0.1991


% Warp

==> sec/Tables/table_3.tex <==
\begin{table*}[t]
\centering
\vspace{-3pt}
\caption{Evaluation Text Prompts for Turbulence Mitigation Learning Guidance}
\label{table:runtime}
\vspace{-2pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}cccccc@{}}
\toprule
 Text Index & Positive Prompts &   Negative Prompt \\ \hline
1 & ``a sharp image"   &   ``a blur image"    \\
2 & ``a sharp image"      & ``a image with blur and turbulence distortion"    \\
3 & ``a clean and sharp natural image"           & ``a degraded image with noise and turbulence distortion"    \\
4 & ``a clean and sharp natural image"    &  ``a degraded image with mosaic and turbulence distortion"    \\
5 & ``a clean and sharp natural image" &  ``a low-resolution image with mosaic and turbulence distortion" \\
6 & ``a clean and sharp natural image with table and alarm clock and books" & ``a low-resolution image with mosaic and turbulence distortion" \\
% BSRN-S-opt(ours)& 156.05     & 8.47     & 184.41  & 26.81  \\
% BSRN(ours)      & 352.405    & 19.44    & 334.17  & 56.93  \\
\bottomrule 

\label{table:clip}
\end{tabular}%
}
\end{table*}
% \vspace{-8pt}  
